Modeling of Interface Loads for EOD Suit Wearers

Explosive Ordnance Disposal (EOD) suits are widely used to protect human operators to execute emergency tasks such as bomb disposal and neutralization. Current suit designs still need to be improved in terms of wearer comfort, which can be assessed based on the interaction forces at the human-suit contact regions. This paper introduces a simulation-based modeling framework that computes the interaction loads at the human-suit interface based on a wearer's kinematic movement data. The proposed modeling framework consists of three primary components: a) inertial and geometric modeling of the EOD suit, b) state estimation of the wearer's in-suit movement, and c) inverse dynamics analysis to calculate the human-suit interface forces based on the simulated human-suit model and the estimated human movement data. This simulation-based modeling method could be used to complement experimental testing for improving the time and cost efficiency of EOD suit evaluation. The accuracy of the simulated interface load was experimentally benchmarked during three different human tasks (each with three trials), by comparing the predicted interface forces with that measured by commercial pressure sensors.

==> excess.tex <==
% There are several advantages of controlling the angular momentum about the contact point (i.e., $L_A$) over the CoM velocity (i.e., $\mathbf{v}_{CoM}$):
% \begin{itemize}
%     \item $L_A$ provides more comprehensive information about the current walking status because it does not only include the linear velocity $\mathbf{v}_{CoM}$, but also the angular momentum of the CoM.
%     \item The derivative of $L_A$ only depends on the CoM position w.r.t the contact point for an under-actuated robot. This means $L_A$ will be weakly affected by the motor peak torque and other disturbances, such as the aggressive motion of a swing leg.
%     \item $L_A$ is invariant if the robot is walking on flat terrain without vertical velocity. On the contrary, the linear velocity $\mathbf{v}_{CoM}$ experiences a jump at the impact based on the impact model, which is always less accurate compared to the continuous model. Using angular momentum about the contact point can help to avoid the inaccuracy that is introduced by the impact model. 
% \end{itemize}


%For simplification purposes, we utilize the sinusoidal wave to represent the DRS motion.



% \begin{itemize}
%     \item Point S: position of the contact point on the DRS w.r.t the wolrd frame.
%     \item Point A: a fixed point that is coincident with the point S at any time in the world frame.
%     \item $\mathbf{p}_{CoM} = [x_c, z_c]\in\mathbb{R}^2$: robot's CoM position in the world frame
%     \item $\mathbf{p}_{SA}=[x_{SA}, z_{SA}]\in\mathbb{R}^2$: position vector from point S to A
% \end{itemize}



% where $\dot{x}_C$ and $\dot{z}_C$ are its horizontal and vertical components.

% := [x_{sc}, z_{sc}]^T\in\mathbb{R}^2
% Note that during regular bipedal walking, the angular momentum $L_{CoM}$ typically oscillates around zero~\cite{9560821}.
% This is because a bipedal robot's trunk is usually built to be substantially heavier than the limbs and the trunk is typically commanded to exhibit negligible angular movement w.r.t. the world frame.

% There are several advantages of controlling the angular momentum about the contact point (i.e., $L_A$) over the CoM velocity (i.e., $\mathbf{v}_{CoM}$)~\cite{9560821}:
% \begin{itemize}
%     \item $L_A$ provides more comprehensive information about the current walking status because it does not only include the linear velocity $\mathbf{v}_{CoM}$, but also the angular momentum of the CoM.
%     \item The derivative of $L_A$ only depends on the CoM position w.r.t the contact point for an under-actuated robot. This means $L_A$ will be weakly affected by the motor peak torque and other disturbances, such as the aggressive motion of a swing leg.
%     \item $L_A$ is invariant if the robot is walking on flat terrain without vertical velocity. On the contrary, the linear velocity $\mathbf{v}_{CoM}$ experiences a jump at the impact based on the impact model, which is always less accurate compared to the continuous model. Using angular momentum about the contact point can help to avoid the inaccuracy that is introduced by the impact model. 
% \end{itemize}
Both original LIP and ALIP suffer accuracy loss from increasing Lc, but ALIP preserves more accuracy as the legs get heavier.

Lc oscillates about zero but I don't think it is always small, Cassie, Digit, mini-cheetah, and Spot have light legs but many other robots have heavy legs. And the legs generate non-negligible Lc when walking.


    % Recently, locomotion on deformable surfaces has been increasingly extensively studied.
    % D. Goldman .et.al investigated the robot locomotion dynamics on granular terrain~\cite{aguilar2016robophysical,li2013terradynamics}. The granular terrain is considered a dynamic surface because the contact between the robot and the surface is subject to significant movement during any step.
    % Later, a model for granular terrain and stability criteria of such locomotion are proposed~\cite{xiong2017stability}, which can guide the control design for a legged robot walking on such terrain with guaranteed stability. 

    % Besides granular terrain, another type of dynamic surface also attracts research interest. Unlike the granular terrain, this type of dynamic surface does not deform but exhibits particular motion w.r.t the world frame. In a real-world application, this type of dynamic surface includes airplanes, ferries, and ground vehicles.
